Randomized Joint Diagonalization of Symmetric Matrices

Given a family of nearly commuting symmetric matrices, we consider the task of computing an orthogonal matrix that nearly diagonalizes every matrix in the family. In this paper, we propose and analyze randomized joint diagonalization (RJD) for performing this task. RJD applies a standard eigenvalue solver to random linear combinations of the matrices. Unlike existing optimization-based methods, RJD is simple to implement and leverages existing high-quality linear algebra software packages. Our main novel contribution is to prove robust recovery: Given a family that is $\epsilon$-near to a commuting family, RJD jointly diagonalizes this family, with high probability, up to an error of norm O($\epsilon$). We also discuss how the algorithm can be further improved by deflation techniques and demonstrate its state-of-the-art performance by numerical experiments with synthetic and real-world data.

==> MEG_runtime_loss.tex <==
\begin{table}[!hbt!]
\begin{center}
\caption{Running time and Loss Comparison for MEG Data}
\begin{tabular}{||c | c | c | |}
\hline
Algorithm Name & Avg Time(ms) & Avg Loss\\
\hline
QNDIAG & $\num{4.995313}$ & $\num{-127.046361}$\\
\hline
PHAM & $\num{272.568892}$ & $\num{-127.046399}$\\
\hline
DRJD & $\num{0.584999}$ & $\num{-126.648748}$\\
\hline
\end{tabular}
\end{center}
\end{table}

==> alternative_exactness_proof.tex <==
\begin{corollary}
With the notation introduced above, let $Q$ be an orthogonal matrix that diagonalizes $A(\mu)$. Then 
$Q$ also diagonalizes each of $A_1,\ldots,A_d$ with probability $1$. 
\end{corollary}
\begin{proof}
The result follows from standard linear algebra arguments \cite{Strang1988}; we include the proof for the sake of completeness.
Without loss of generality, we may assume that the first $n_1 \ge 1$ columns of $Q$ span an eigenspace 
$\mathcal X_1$ belonging to an eigenvalue $\lambda_1(\mu)$ of $A(\mu)$. Then
\[
Q^T A(\mu) Q = \begin{bmatrix}
 \lambda_1(\mu) I & 0 \\
 0 & A_{22}(\mu)
 \end{bmatrix}, \quad Q^T A_k Q
= \begin{bmatrix}
 A_{11}^{(k)} & \big( A_{21}^{(k)} \big)^T \\
 A_{21}^{(k)} & A_{22}^{(k)}
 \end{bmatrix}.
\]
Because $A(\mu)$ and $A_k$ commute, one has $(A_{22}(\mu) - \lambda_1(\mu))A_{21}^{(k)} = 0$ and, together with $\lambda_1(\mu) \not\in A_{22}(\mu)$, this implies $A_{21}^{(k)} = 0$. By  Lemma~\ref{lemma:multieigenvalues}, $A_{11}^{(k)}$ has $n_1$ equal eigenvalues with probability $1$ and is, in turn, a multiple of the identity matrix. This completes the proof by induction.
\end{proof}

\begin{theorem} \label{thm:exactlycommuting}
Given a commuting family of  symmetric matrices $\{A_k\}_{k = 1}^d$, let 
 $Q$ be an orthogonal matrix that diagonalizes $A(\mu) = \mu_1 A_1 + \cdots + \mu_d A_d$ for $\mu \sim \mathcal N(0,I_d)$. Then, with probability $1$, 
$Q$ also diagonalizes each of $A_1,\ldots,A_d$. 
\end{theorem}
\begin{proof}
Considering an arbitrary eigenvector $v$ of $A(\mu)$, we have 
\[A(\mu) v = \lambda(\mu)v = \mu_1\lambda_1v + \dots + \mu_d\lambda_dv.\]
After rearrangement, this yields
\[\mu_1 (A_1 - \lambda_1I) v + \dots + \mu_d (A_d - \lambda_dI) v = 0.\]
Since there is zero probability for $\mu_k = 0$ for any $k$, we have
\[(A_k - \lambda_kI)v = 0, \quad k = 1,\ldots,d.
\]
with probability $1$.
\textcolor{red}{There is a problem with this line of argument!!! Each $v$ is considered deterministic in the above argument, but in the final conclusion it is not. $Q$ and hence $v$ depend on $\mu$!}
Therefore, $Q$ will be a matrix whose columns are eigenvectors for each $A_k, k \in \{1,\ldots,d\}$, which completes the proof.
\end{proof}

\begin{comment}\begin{algorithm}[H]
\caption{Clustering}
\textbf{Input:}$\Lambda_1,\ldots,\Lambda_n$\\
 \textbf{Output:} Clustering $K$.
\begin{algorithmic}
\label{alg:cluster}
\STATE k = 1
\REPEAT
\STATE Let $i$ be the first one that $K(i)$ is not assigned yet, let $K(i) = k$.
\REPEAT
\FOR{$j=1$ to $n$}
    \IF{$K(j)$ is unassigned and $\exists l$ such that $K(l) = k$ and $\eunorm{\Lambda_l - \Lambda_j} \leq \delta$}
    \STATE Let $K(j) = k$
    \ENDIF
\ENDFOR
\UNTIL There is no more $i \in \{1,\ldots, n\}$ that we can let $K(i) = k$.
\STATE k = k + 1
\UNTIL There is no  $i \in \{1,\ldots, n\}$ that does not have a value $K(i)$.
\RETURN K
\end{algorithmic}
\end{algorithm}
\end{comment}

==> non_asymtotic.tex <==
\section{Non-asymptotic Result}

Reminder for myself ($=$ DK):
\begin{itemize}
    \item Are exactness results also phrased in terms of eigenspaces?
    \item kernel already defined?
    \item Clarify somewhere that ``is a basis'' means columns of ... form a basis.
\end{itemize}

Reminders for myself: Recall definition of $\Lambda_i$.
\begin{lemma}\label{Perturbation Analysis}
Let $A,E \in \reals^{n \times n}$ be symmetric with $\fnorm{E} = \epsilon$. For an eigenvalue $\lambda_0$
 of $A$, we let 
$s_0 := \min\{\abs{\lambda_0 -\nu}: \nu \in \sigma(A) \setminus \{\lambda_0\}\}$ denote the separation of $\lambda_0$ and assume that $\epsilon  < s_0/4$. Considering the eigenspace $\mathcal{X}_0= \kernel(\lambda_0 I-A)$, the perturbed matrix $A+E$ has a unique invariant subspace
$\mathcal{X}_E$ of the same dimension such that the corresponding eigenvalues are contained in the interval $[\lambda_0 - \epsilon, \lambda_0 + \epsilon]$. Moreover,
for any orthonormal basis $X_E$ of $\mathcal{X}_E$, there exists a basis $\hat  X_0$ of $\mathcal{X}_0$ and a matrix $B$ such that 
\[
    X_E = \hat X_0  + (\lambda_0 I - A)\pesudoinverse B, \quad \fnorm{B} \leq \sqrt{5}\fnorm{EX_0}.
\]
\end{lemma}
\begin{proof}
The result follows from existing perturbation results on invariant subspaces~\cite{StewartSun1990,MR3205738}. We may assume without loss of generality that 
\[ A = \begin{bmatrix}
\lambda_0I & 0 \\ 0 & A_{22}
\end{bmatrix}, \mspace{10mu} \lambda_0 \not\in \sigma(A_{22}), \mspace{10mu} E =  \begin{bmatrix}
E_{11} & E_{12} \\  E_{21} & E_{22}
\end{bmatrix}.\]
Note that $X_0 = \begin{bmatrix}
I \\ 0
\end{bmatrix}$ is an orthonormal basis of $\mathcal X_0$ and $\hat{X}_E = \begin{bmatrix}
I \\ W_E
\end{bmatrix}$ spans an invariant subspace $\mathcal{X}_E$  of $A+E$ if and only if $W_E$ satisfies
\begin{equation} \label{eq:quadmateq}
(\lambda_0 I - A_{22}) W_E = 
\begin{bmatrix}
 -W_E & I
\end{bmatrix}E
\begin{bmatrix}
 I \\
 W_E
\end{bmatrix}.
%E_{21} + E_{22}W_E - W_E E_{11} - W_EE_{12}W_E;
\end{equation}
Theorem 3.1 in~\cite{MR3205738} and Theorem 2.7 in~\cite{StewartSun1990}
show that this quadratic matrix equation admits a unique solution $W_E$ satisfying the bounds
\[
\fnorm{W_E} \le \frac{2}{s_0}\fnorm{E} \leq \frac{1}{2}, \quad
\fnorm{W_E} \leq \frac{2}{s_E}\fnorm{E_{21}},
\]
respectively, where $s_E := s_0 - \fnorm{E_{11}} - \fnorm{E_{22}} > 2\epsilon$. Theorem 3.1 in \cite{MR3205738} also shows that the eigenvalues of $A+E$ corresponding to $\mathcal{X}_E$ are in $[\lambda_0 - \epsilon, \lambda_0 + \epsilon]$ and, by the assumption on $\epsilon$, no other eigenvalue can be contained in that interval.
Using~\eqref{eq:quadmateq}, we thus obtain
\begin{align*}
\|(\lambda_0 I - A_{22}) W_E\|_F \leq& \left\| \begin{bmatrix}
 -W_E & I
\end{bmatrix} \right\|_2 \cdot \left\| E
\begin{bmatrix}
 I \\
 W_E
\end{bmatrix}\right\|_F \le \frac{\sqrt{5}}{2} \left\| E
\begin{bmatrix}
 I \\
 W_E
\end{bmatrix}\right\|_F \\ \le&  \frac{\sqrt{5}}{2} \left( \|E X_0\|_F + \left\| E
\begin{bmatrix}
 0 \\
 W_E
\end{bmatrix}\right\|_F  \right) 
\le \frac{\sqrt{5}}{2} \left( \|E X_0\|_F + \frac{2\epsilon }{s_E} \|E_{21}\|_F \right) \\
\le & \sqrt{5} \|E X_0\|_F.
\end{align*}
 We obtain a (particular) orthonormal basis $\tilde X_E$ of $\mathcal X_E$ by setting
\[
\tilde{X}_E := \hat X_E ( I + W_E^T W_E)^{-1/2} = \hat X_0 + (\lambda_0 I - A)\pesudoinverse B 
\]
with
\[
\hat X_0 = X_0 ( I + W_E^T W_E)^{-1/2}, \quad B = 
\begin{bmatrix}
 0 \\
 (\lambda_0 I - A_{22}) W_E
\end{bmatrix}
( I + W_E^T W_E)^{-1/2}
\]
Because of $I \gtrsim ( I + W_E^T W_E)^{-1/2}$ 
\textcolor{blue}{??? If I understand your proof correctly, does the symbol mean the ordering introduced by PSD cone, and I am wondering should we introduce it somewhere in our notation section or here. ???}, it follows from matrix monotonicity that $\fnorm{B} \leq \|(\lambda_0 I - A_{22}) W_E\|_F \le \sqrt{5} \|E X_0\|_F$. This completes the proof, using that any other orthonormal basis $X_E$ of $\mathcal X_E$ is related to $\tilde X_E$ via an orthonormal change of basis.
\end{proof}

\textcolor{blue}{
EXPLANATIONS for the old proof:
\begin{itemize}
    \item $\|Z_i\|_F \le 1/2$ is coming from the bound of $W_E$ inside Lemma 5, which is not covered by Lemma 5. It is used to bound 
    $$\fnorm{E_k\tilde{X}} = \fnorm{E_k(Y + Z)}.$$
    where
    \[\tilde{X}=\begin{bmatrix}
\tilde{X}_1 & \dotsb & \tilde{X}_m \end{bmatrix},\]
\[Y=\begin{bmatrix}
Y_1 & \dotsb & Y_m \end{bmatrix}\]
and 
\[Z=\begin{bmatrix}
Z_1 & \dotsb & Z_m \end{bmatrix}.\]
    But it is not needed at all because
    $$\fnorm{E_k\tilde{X}} \leq \fnorm{E_k}$$
    for $\tilde{X}$ is an orthonormal basis of $\reals^n$. Sorry for making it unnecessarily complicated!
\item Since $\tilde{Q}$ diagonalizes $\tilde{A}(\mu)$, $\tilde{A}(\mu)$ is symmetric and each perturbed invariant subspace $\tilde{\mathcal{X}}_i$ has distinct spectrum, we have that $\tilde{Q} = \begin{bmatrix}
\tilde{X}_1 \ldots \tilde{X}_m 
\end{bmatrix}$ where each $\tilde{X}_1$ consists of bases  for perturbed eigenspaces inside each perturbed invariant subspace $\tilde{\mathcal{X}}_i$, and therefore $\tilde{X}_i$ is also an orthornormal basis for perturbed invariant subspace $\tilde{\mathcal{X}}_i$. By Lemma \ref{Perturbation Analysis} (holds for any orthornormal basis of the perturbed invariant subspace), we can get 
\[\tilde{X}_i = Y_i + (\lambda(\mu) - A(\mu))\pesudoinverse B.\]
\end{itemize}
}

\begin{theorem}
\label{main theorem}
Suppose $\Acal = \{A_k \in \reals^{n \times n}\}_{k=1}^{d}$ is an exactly commuting family. Suppose that there are symmetric matrices $E_k \in \reals^{n \times n}, k \in \{1,\dots,d\}$  such that $\sum_{k=1}^{d}\fnorm{E_k}^2 \leq \epsilon^2$. Let $\tilde{\Acal} = \{\tilde{A_k} = {A_k} + E_k\}$ for $k \in \{1,\dots,d\}$. Let $\Vec{\mu} \sim \mathcal{N}(0, I_d)$ be a standard normal random vector and consider the corresponding linear combination $\tilde{A}(\Vec{\mu}) = \sum_{k=1}^{d} \mu_k\tilde{A_k}$, with $A(\Vec{\mu}), E(\Vec{\mu})$ defined analogously.
 Let $m$ be the number of mutually distinct eigenvalues of $\Acal$. Let $s = \min_{i \neq j}\| \Vec{\Lambda}_i - \Vec{\Lambda}_j\|_2$ be the minimal gap of eigenvalue vectors. For $\epsilon > 0$, if $\tilde{Q} \in \reals^{n \times n}$ such that $\tilde{Q}^T \tilde{Q} = I_n$ and  $\tilde{Q}^T\tilde{A}(\Vec{\mu})\tilde{Q}$ is diagonal, then
\[\Prob\Big(\sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2 \leq R^2 \epsilon^2  \Big)\geq \begin{cases}
1 - 3\frac{dm(m-1)}{\sqrt{2\pi}(R-1)}, &\text{for } 1 < R  \leq \frac{3\sqrt{d}s}{4\epsilon}+ 1 \\
1 -\frac{4\sqrt{d}m(m-1)\epsilon}{\sqrt{2\pi}s}, &\text{for } R  > \frac{3\sqrt{d}s}{4\epsilon}+ 1.

\end{cases}
\]
\end{theorem}
\begin{proof}
Let $\lambda_1(\mu),\ldots,\lambda_m(\mu)$ denote the mutually distinct eigenvalues of $A(\mu)$ and let $n_i$ denote the multiplicity of $\lambda_i(\mu)$. By Lemma~\ref{lemma:multieigenvalues}, the $n_i$ eigenvalues of $A_k$ belonging to $\lambda_i(\mu)$ are all equal (with probability 1) to the same number $\lambda_i^{(k)}$. By letting $\Lambda_i = [\lambda_i^{(1)}, \ldots, \lambda_i^{(d)}]$, we can write $\lambda_i(\mu) = \langle \mu, \Lambda_i \rangle$.

We now assume that 
\begin{equation}\label{eq:eigengap_assum}
    \fnorm{E(\Vec{\mu})} \leq \frac{\inner{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\Vec{\mu}}}{4} , \quad \forall i \neq j.
\end{equation}
%Let $X_i$ form an orthonormal basis for the eigenspace $\mathcal{X}_i$ belonging to the eigenvalue $\lambda_i(\Vec{\mu})$ of $A(\mu)$.
This assumption allows us to apply Lemma~\ref{Perturbation Analysis} to each eigenspace $\mathcal X_i = \kernel(\lambda_i(\Vec{\mu})I - A(\Vec{\mu}))$ and conclude that, after a suitable permutation of its columns, the matrix $\tilde Q$ takes the form
\[
\tilde Q = [\tilde X_1,\ldots,\tilde X_m]
\]
with
\[
\tilde{X}_i = \hat Y_i + (\lambda_i(\Vec{\mu})I - A(\Vec{\mu})) B_i
\]




exists a basis $\hat{X}_1$ of an invariant subspace $\tilde{\mathcal{X}}_1$ of $\tilde{A}(\Vec{\mu})$ such that
\[
(\hat{X_1} - X_1)^TX_1 =\textbf{0}, \quad 
\hat{X}_1 =  X_1 + (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_1
\]
for some matrix $B_1$ with $B_1 \leq \sqrt{5} \fnorm{E(\Vec{\mu})X_1}$.
\textcolor{red}{%Remarks:
%\begin{itemize}
    %\item The orthogonalization stuff should be covered in Lemma 5. Think carefully about what you need exactly and prove it properly. Basically, you seem to replace $Z$ by $Z (I+Z^T Z)^{-1/2}$ and then you upper bound (like sin is bounded by tan) but this does not come out very clearly. It will be much easier to state/prove within the proof of the lemma.
    %\item You need to provide a more specific argument/reference why the perturbed invariant subspaces stay distinct.
    %\item I don't see where $\|Z_i\|_F \le 1/2$ is coming from (and whether it is actually used). You are not allowed to use facts established inside a proof without mentioning it. (And even if you mention it, it bad practice and should be avoided whenever possible.)
    %\item ``without loss of generality, we can assume $\tilde{Q}...$'' there are quite some steps needed to see this. especially why can you assume that $\tilde X_1$ is the correct choice for the (perturbed) eigenspace? Either find a compact argument or allow for a small orthogonal transformation of each block column and deal with it later.
%\end{itemize}
}


Some new snippets (please ignore):
\begin{align}
        \| \offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q}) \|_F^2 \le & 
        \big\| \tilde{Q}^T\tilde{A}_k\tilde{Q} - \text{diag}\big(\lambda^{(k)}_1 I_{n_1}, \ldots, \lambda^{(k)}_m I_{n_m}\big)  \big\|_F^2  \nonumber \\ 
        = & \big\| \tilde{A}_k\tilde{Q} -  \tilde{Q}\, \text{diag}\big(\lambda^{(k)}_1 I_{n_1}, \ldots, \lambda^{(k)}_m I_{n_m}\big)  \big\|_F^2      \label{eq:offdiag_errornew} \\
        =& \big\| ( \tilde{A}_k - \lambda^{(k)}_1 I ) \tilde X_1\big\|_F^2 + \cdots + 
        \big\| ( \tilde{A}_k - \lambda^{(k)}_m I ) \tilde X_m \big\|_F^2. \nonumber
\end{align}

OLD PROOF STARTS HERE:

Let $\{\Vec{x}_1,...,\Vec{x}_n\}$ be an orthonormal basis consisting of common eigenvectors for $\{A_k\}_{k=1}^d$. Let $\lambda_{ki}$ be the eigenvalue of $x_i$ for the matrix $A_k$ for $i \in [n], k \in \{1,\dots,d\}$. Let $m$ (the number of ``groups" of eigenvalues), $\{n_1,\dots,n_{m+1}\}$, the matrix $\Lambda $ and its columns $\Vec{\Lambda}_i$'s be defined as in Section \ref{subsec:exact_correct}. Then by Lemma \ref{lemma:multieigenvalues}, we know that $A(\mu)$ will share the same $m$ ``groups" of eigenvalues as $A_1,\dots,A_d$, that is, $\lambda_i(\Vec{\mu}) = \lambda_{n_r}(\Vec{\mu}) $ for all $i \in [n_{r},n_{r+1}), r \in \{1,\dots,m\}$,  and for $i,j \in \{1,\dots,m\}$, if $i \neq j$, then $\lambda_{n_i}(\Vec{\mu})  \neq  \lambda_{n_j}(\Vec{\mu})$ with probability $1$. 

We first assume that $\fnorm{E(\Vec{\mu})}$ is smaller than one forth of the minimal eigengap of $A(\mu)$, that is,
\begin{equation}\label{eq:eigengap_assum}
    \fnorm{E(\Vec{\mu})} \leq \frac{\inner{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\Vec{\mu}}}{4} , \forall i \neq j,
\end{equation}
so that we can apply the eigenspace perturbation lemma.

Consider the random linear combination $\tilde{A}(\Vec{\mu}) = A(\Vec{\mu}) +  E(\Vec{\mu})$. Without loss of generality again,  we consider the first group of eigenvectors. Let matrix $X_1 = \begin{bmatrix} \Vec{x}_1 & \Vec{x}_2 & \dotsb &  \Vec{x}_{n_1-1} \end{bmatrix}$, columns of $X_1$ form an orthonormal basis for the eigensapce $\mathcal{X}_1$ of $\lambda_1(\Vec{\mu})$ for $A(\Vec{\mu})$ with probability $1$. By Lemma \ref{Perturbation Analysis} there exists $\hat{X}_1$ such that:
\begin{enumerate}[label=(\roman*)]
    \item Columns of $\hat{X}_1$ form a basis of an invariant subspace $\tilde{\mathcal{X}}_1$ of $\tilde{A}(\Vec{\mu})$.
    \item For all square matrix $C$ with compatible dimension, because the residual is perpendicular, that is, $(\hat{X_1} - X_1)^TX_1 =\textbf{0} $,  we have $\eunorm{X_1C} \leq \eunorm{\hat{X}_1C}$.
    \item $\hat{X}_1 =  X_1 + (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B(\Vec{\mu})$ where $\fnorm{B(\Vec{\mu})} \leq 3\fnorm{E(\Vec{\mu})X_1}$. 
\end{enumerate}
   
For any $\tilde{X}_1$ which is an orthonormal basis of $\tilde{\Xcal}_1$, there exist a square matrix $C_1$ with compatible dimension such that $\tilde{X}_1 = \hat{X}_1 C_1$, and $\eunorm{C_1}\leq 1$. Thus, we have that
\[
    \tilde{X}_1 = Y_1 + (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_1(\Vec{\mu})C_1
\]
where $Y_1 = X_1 C_1$ with $\eunorm{Y_1} \leq \eunorm{\tilde{X}_1} = 1$ and $\fnorm{B(\Vec{\mu})C_1} \leq 3\fnorm{E(\Vec{\mu})X_1} $. Since $\Col(Y_1)$ is at least a subspace of $\mathcal{X}_1$, which corresponds to the first group of eigenvalues, we have $(A_k - \lambda_{k1}I)Y_1 = 0$ for all $k \in \{1,\dots,d\}$.

The above argument works for any $X_i$ which is an orthonormal basis for $\Xcal_i$ for $i \in \{1,\dots,m\}$. Thus, for $i \in \{1,\dots,m\}$, with  $\tilde{\mathcal{X}}_i$ defined as above, for any $\tilde{X}_i$ which is an orthonormal basis of $\tilde{\Xcal}_i$, we have that
\begin{equation}
\label{eq:linearization}
    \tilde{X}_i =  Y_i + (\lambda_{n_i}(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_i(\Vec{\mu})C_i
\end{equation} 
where $\eunorm{Y_i} \leq 1$, $\fnorm{B(\Vec{\mu})} \leq 3\fnorm{E(\Vec{\mu})X_i} $ and $(A_k - \lambda_{kn_i}I)Y_i =0$ for all $k \in \{1,\dots,d\}$.

For the invariant subspaces $\tilde{\Xcal}_i$'s, as the eigenvalues belonging to different $\tilde{\Xcal}_i$'s do not overlap, and the matrix $\tilde{A}(\Vec{\mu})$ is symmetric, we have that \[\tilde{\Xcal}_i \perp \tilde{\Xcal}_j, \forall i \neq j\] 
and 
\[\bigoplus_{i=1}^{m} \tilde{\Xcal}_i = \reals^n.\] 
In turn, without loss of generality, we can assume $\tilde{Q}= \begin{bmatrix}
\tilde{X}_1 & \dotsb & \tilde{X}_m \end{bmatrix}$.

If we view $\tilde{X}_i$ as an orthonormal basis of an approximated eigenspace of $\tilde{A}_k$ with an approxiamted eigenvalue $\lambda_{kn_i}$,  $(\tilde{A}_k - \lambda_{kn_i}I)\tilde{X}_i$ can be thought of as the residual.  Then from (\ref{eq:linearization}), we get for any $k \in \{1,\dots,d\}, i \in \{1,\dots,m\}$, the residual $(\tilde{A}_k - \lambda_{kn_i}I)\tilde{X}_i$ is small  as shown below:
\begin{equation}
\label{eq:residue}
    \begin{split}
         (\tilde{A}_k - \lambda_{kn_i}I)\tilde{X}_i &= (A_k - \lambda_{kn_i}I + E_k )(Y_i + Z_i) \\
         &=  (A_k - \lambda_{kn_i}I) (\lambda_{n_i}(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B(\Vec{\mu})C_i +E_k(Y_i + Z_i)
    \end{split}
\end{equation}
where 
\[Z_i = (\lambda_{n_i}(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_i(\Vec{\mu})C_i\]
and
\[\fnorm{Z_i} \leq \frac{1}{2}\]
In turn, small residue can imply small off-diagonal error.
For any $i\in \{1,\dots,m\}$, consider the $i$-th group of columns in $\tilde{Q}^T\tilde{A}_k\tilde{Q}$ for any $k \in \{1,\dots,d\}$,
\[
    \tilde{Q}^T\tilde{A}_k\tilde{X}_i = \tilde{Q}^T(\tilde{A}_k - \lambda_{kn_i}I)\tilde{X}_i + \lambda_{kn_i}\tilde{Q}^T \tilde{X}_i.
\]
Notice that the entries in $\lambda_{kn_i}\tilde{Q}^T \tilde{X}_i$ that corresponds to the off-diagonal entries of $\tilde{Q}^T\tilde{A}_k\tilde{Q}$ are all zero. Thus, we have
\begin{equation}
    \label{eq:offdiag_error}
    \begin{split}
        &\fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2\\
        \leq&{} \fnorm{\begin{bmatrix} \tilde{Q}^T(\tilde{A}_k - \lambda_{k1}I)\tilde{X}_1 &\dotsb & \tilde{Q}^T(\tilde{A}_k - \lambda_{km}I)\tilde{X}_m\end{bmatrix}}^2\\
        =&{} \fnorm{\begin{bmatrix} (\tilde{A}_k - \lambda_{k1}I)\tilde{X}_1 &\dotsb &(\tilde{A}_k - \lambda_{km}I)\tilde{X}_m\end{bmatrix}}^2.
    \end{split}
\end{equation}
By (\ref{eq:residue}), we have
\[
\begin{split}
    &\begin{bmatrix} (\tilde{A}_k - \lambda_{k1}I)\tilde{X}_1 &\dotsb &(\tilde{A}_k - \lambda_{km}I)\tilde{X}_m\end{bmatrix} \\
    =&{} \begin{bmatrix} (A_k - \lambda_{k1}I) (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_1(\Vec{\mu})C_1 &\dotsb & (A_k - \lambda_{kn_m}I) (\lambda_m(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_m(\Vec{\mu})C_m\end{bmatrix} \\
    & + E_k \tilde{X}.
\end{split}
\]
where
\[\tilde{X}=\begin{bmatrix}
\tilde{X}_1 & \dotsb & \tilde{X}_m \end{bmatrix}\]
\begin{equation}
\label{eq:error_split}
\begin{split}
    &\fnorm{\begin{bmatrix} (\tilde{A}_k - \lambda_{k1}I)\tilde{X}_1 &\dotsb &(\tilde{A}_k - \lambda_{km}I)\tilde{X}_m\end{bmatrix}}  \\
    \leq&{} \fnorm{\begin{bmatrix} (A_k - \lambda_{k1}I) (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_1(\Vec{\mu}) &\dotsb & (A_k - \lambda_{kn_m}I) (\lambda_m(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_m(\Vec{\mu})\end{bmatrix}}\\
    &+\fnorm{E_k}.
\end{split}
\end{equation}
Next, let 
\[C_{max}(\Vec{\mu}) = \max_{i \in \{1,\dots,m\}, k \in \{1,\dots,d\}}\{\eunorm{ (A_k - \lambda_{kn_i}I) (\lambda_{i}(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse }\}.\]
Then, 
\begin{equation}
\label{eq:first_error_term}
\begin{split} 
&\fnorm{\begin{bmatrix} (A_k - \lambda_{k1}I) (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_1(\Vec{\mu}) &\dotsb & (A_k - \lambda_{kn_m}I) (\lambda_m(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_m(\Vec{\mu})\end{bmatrix}}^2\\
    =&{}\sum_{i=1}^{m}\fnorm{(A_k - \lambda_{kn_i}I) (\lambda_i(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse B_i(\Vec{\mu})}^2\\
    \leq&{}\sum_{i=1}^{m}\eunorm{(A_k - \lambda_{kn_i}I) (\lambda_i(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse}^2 \fnorm{ B_i(\Vec{\mu})}^2\\
    \leq&{}9\sum_{i=1}^{m}C_{max}(\Vec{\mu})^2\fnorm{E(\Vec{\mu})X_i}^2\\
    \leq&{} 9C_{max}(\Vec{\mu})^2 \fnorm{ E(\Vec{\mu})}^2.\\
\end{split}
\end{equation}
Thus, combining (\ref{eq:offdiag_error}) (\ref{eq:error_split}) and (\ref{eq:first_error_term}),
\begin{equation}
    \fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2 \leq  9C_{max}(\Vec{\mu})^2 \fnorm{E(\Vec{\mu})}^2 + 6C_{max}(\Vec{\mu})\fnorm{E(\Vec{\mu})}\fnorm{E_k}  + \fnorm{E_ k}^2.
\end{equation}
Then
\begin{equation}
\begin{split}
    &\sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T \tilde{A}_k \tilde{Q})}^2\\
    \leq&{} 9dC_{max}(\Vec{\mu})^2 \fnorm{E(\Vec{\mu})}^2 + 6\sqrt{d}C_{max}(\Vec{\mu})\fnorm{E(\Vec{\mu})}\epsilon^2  +  \epsilon^2\\
    \leq&{} ( 1 + 3\sqrt{d}C_{max}(\Vec{\mu})\eunorm{\Vec{\mu}})^2\epsilon^2.
\end{split}
\end{equation}
The last inequality follows from $\eunorm{E(\Vec{\mu})}^2 \leq \eunorm{\Vec{\mu}}^2 \epsilon^2$ by Cauchy-Schwarz Inequality. Furthermore, if we assume \[C_{max}(\Vec{\mu})\eunorm{\Vec{\mu}} \leq \frac{(R-1)}{3\sqrt{d}},\] we have
\begin{equation}
    \label{eq:finalerror}
 \sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T \tilde{A}_k \tilde{Q})}^2\leq  R^2\epsilon^2.
 \end{equation}
Therefore, we would like to consider the random variable
\[X = \max_{i \in \{1,\dots,m\}, k \in \{1,\dots,d\}}\{\eunorm{ (A_k - \lambda_{kn_i}I)
(\lambda_{i}(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse }\eunorm{\Vec{\mu}}\}.\]
We want the event $X < (R-1)/3\sqrt{d}$ to happen. Hence, we consider the failure probability
\begin{equation}
\label{eq:failure_event_1}
    \begin{split}
            Pr\big( \exists i \in \{1,\dots,m\}, \exists k \in \{1,\dots,d\}, \eunorm{ (A_k - \lambda_{kn_i}I) (\lambda_i(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse}\eunorm{\Vec{\mu}}  \geq \frac{R-1}{3\sqrt{d}}\big).
    \end{split}
\end{equation}
Without loss of generality, we look at the matrix $(A_k - \lambda_{k1}I) (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse$ corresponding to the first ``group" of eigenvalues. Denote its $i$-th eigenvalues by $\alpha_{ki}$, we have
\[\alpha_{ki} = 
    \begin{cases}
    0, &  \lambda_{ki} = \lambda_{k1}, \\
    -(\lambda_{ki}- \lambda_{k1}) / \inner{\Vec{\Lambda }_i -\Vec{\Lambda}_1}{\Vec{\mu}}=-1 / \inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{(\lambda_{ki}- \lambda_{k1})}}{\Vec{\mu}}, & \lambda_{ki} \neq \lambda_{k1}.
    \end{cases}
\]
Notice that for each $i$, since $\lambda_{ki} - \lambda_{k1}$ is not random, there exists a fixed $k_{max}(i)$ such that $\abs{\alpha_{k_{max}(i)i}}$ is the maximum among $\{\abs{\alpha_{ki}},i \in {1,\dots,d}\}$. Thus,
\begin{equation}
\label{eq:failure_event_2}
\begin{split}
    &Pr\big(\exists k \in \{1,\dots,d\}, \eunorm{ (A_k - \lambda_{kn_1}I) (\lambda_1(\Vec{\mu})I - A(\Vec{\mu}))\pesudoinverse}\eunorm{\Vec{\mu}}  \geq \frac{R-1}{3\sqrt{d}}\big)\\
    =&{}Pr\big(\exists i \in [n], \abs{\alpha_{k_{max}(i)i}}\eunorm{\Vec{\mu}} \geq \frac{R-1}{3\sqrt{d}}\big).
\end{split}
\end{equation}
If $\alpha_{ki} \neq 0$, we have for any $i \in \{1,\dots,n\}$,
\[ -\frac{1}{\alpha_{ki}} = \inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\lambda_{ki}- \lambda_{k1}}}{\Vec{\mu}}. \]
Then consider $1 / (\abs{\alpha_{ki}}\eunorm{\Vec{\mu}})$,
\[\frac{1}{\abs{\alpha_{ki}}\eunorm{\Vec{\mu}}} = \abs{\inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\lambda_{ki}- \lambda_{k1}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}}}.\]
It is a well-known fact that normalized Gaussian vector $\Vec{\mu}/\eunorm{\Vec{\mu}}$ follows a uniform distribution over the unit sphere. And notice that 
\begin{equation}
    \label{eq:norm_bigger_than_one}
    \eunorm{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\lambda_{ki}- \lambda_{k1}}} \geq 1
\end{equation} for $i$ such that $\lambda_{ki} \neq \lambda_{k1}$. Therefore,
\begin{equation}
\label{eq:probability_for_one_eigenvalue}
\begin{split}
   Pr\big(\abs{\alpha_{ki}}\eunorm{\Vec{\mu}} \geq \frac{R-1}{3\sqrt{d}}\big) &= Pr\big(\abs{\frac{1}{\alpha_{ki}\eunorm{\Vec{\mu}}}} \leq \frac{3\sqrt{d}}{R-1}\big)\\
    &= Pr\big( \abs{\inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{(\lambda_{ki}- \lambda_{k1})}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}}} \leq \frac{3\sqrt{d}}{R-1}\big)\\
    &= Pr\big( \abs{\inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_1}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}}} \leq \frac{3\sqrt{d}}{(R-1)\eunorm{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\lambda_{ki}- \lambda_{k1}}}}\big)\\
    &\leq Pr\big( \abs{\inner{\frac{\Vec{\Lambda}_i -\Vec{\Lambda}_1}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_1}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}}} \leq \frac{3\sqrt{d}}{R-1}\big) \\
    &\leq \sqrt{\frac{2}{\pi}}\frac{3d}{R-1}.
\end{split}
\end{equation}
The second last inequality follows from (\ref{eq:norm_bigger_than_one}), and the last inequality stems from   Lemma \ref{Probability Bound}. From the derivation we see that to bound each 
\[Pr(\abs{\alpha_{k_{max}(i)i}}\eunorm{\Vec{\mu}} \geq \frac{(R - 1)}{3\sqrt{d}}),\]
we need to bound the inner product between $\Vec{\mu}/\eunorm{\Vec{\mu}}$ and $(\Vec{\Lambda}_i - \Vec{\Lambda}_1)/\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_1}$ (for each event we need to bound along the direction $\Vec{\Lambda}_i - \Vec{\Lambda}_1$). But we have overall at most $\binom{m}{2} = m(m-1)/2$ different directions to consider for \[\Vec{\Lambda}_{n_i} - \Vec{\Lambda}_{n_j}, i,j \in \{1,\dots,m\} \wedge i \neq j.\] Thus, by applying a union bound with (\ref{eq:probability_for_one_eigenvalue}) to (\ref{eq:failure_event_2}) we have
\begin{equation}
    \label{eq:failure_probability}
    Pr(X \geq \frac{R-1}{3\sqrt{d}})) \leq \frac{3dm(m-1)}{\sqrt{2\pi}(R-1)} .
\end{equation}
Combining (\ref{eq:finalerror}) and (\ref{eq:failure_probability}), we get
\[ Pr\big( \sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T \tilde{A}_k \tilde{Q})}^2\leq R^2\epsilon^2 \big) \geq 1 -  \frac{3dm(m-1)}{\sqrt{2\pi}(R-1)}.\]

All the above argument is based on the assumption (\ref{eq:eigengap_assum}). We would like to derive a sufficient condition such that (\ref{eq:eigengap_assum}) holds. We have
\[\fnorm{E(\Vec{\mu})} \leq \eunorm{\Vec{\mu}}\epsilon.\]
Therefore, we want
\begin{equation}
    \label{eq:gap}
    \forall i \neq j, \inner{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}} \geq 4\epsilon.
\end{equation}

Modify (\ref{eq:gap}) a bit, we have
\begin{equation}
    \forall i \neq j, \inner{\frac{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}} \geq \frac{4\epsilon}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}}. 
\end{equation}
Thus, Let $s = \min_{i \neq j}\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}$, we only need the event
\begin{equation}
    \label{eq:gap_m}
    \forall i \neq j, \inner{\frac{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}} \geq \frac{4\epsilon}{s}.
\end{equation}
In our probabilistic perturbation analysis, we need the event
\begin{equation}
    \label{eq:failure_prob}
    \forall i \neq j, \inner{\frac{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}} \geq \frac{3\sqrt{d}}{R-1}.
\end{equation}

 Compare (\ref{eq:failure_prob}) with (\ref{eq:gap_m}), we find out that if 
\[R \leq \frac{3}{4}\frac{s}{\epsilon}\sqrt{d} + 1,\] 
We have the event (\ref{eq:gap_m}) automatically. That is, for small error tolerance $R$, $R  \leq 3s\sqrt{d}/\epsilon + 3/2$, our previous probability bound still applies. For $R  > 3s\sqrt{d}/4\epsilon + 3/2$, we need only (\ref{eq:gap_m}). Similarly, the probability will be
\[ P \big(\forall i \neq j, \inner{\frac{\Vec{\Lambda}_i - \Vec{\Lambda}_j}{\eunorm{\Vec{\Lambda}_i - \Vec{\Lambda}_j}}}{\frac{\Vec{\mu}}{\eunorm{\Vec{\mu}}}} \geq \frac{4\epsilon}{s} \big) \geq  \frac{4\sqrt{d}m(m-1)\epsilon}{\sqrt{2\pi}s}. \]

Overall, if $R \leq \frac{3}{4}\frac{s}{\epsilon}\sqrt{d} + 1$,
\[Pr\big(\sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2 \leq R^2 \epsilon^2  \big)\geq 1 - 3\frac{dm(m-1)}{\sqrt{2\pi}(R-1)}.\]
If $ R > \frac{3}{4}\frac{s}{\epsilon}\sqrt{d} + 1$,
\[Pr\big(\sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2 \leq R^2 \epsilon^2  \big) \geq 1 -  \frac{4\sqrt{d}m(m-1)\epsilon}{\sqrt{2\pi}s}.\]
\end{proof}
\begin{remark}
If we instead use asymptotic invariant subspace perturbation result, e.g. \cite[Lemma 2.3]{MR3205738}, and follow the same proof strategy of the non-asymptotic probabilistic bound without the argument of controlling the eigenvalue gap of $A(\Vec{\mu})$, the result will have a better constant as follows:
for $R>1$,
\[\Prob\big(\sum_{k=1}^{d}\fnorm{\offdiag(\tilde{Q}^T\tilde{A}_k\tilde{Q})}^2 \leq R^2 \epsilon^2 + \Ocal(\epsilon^3)\big) \geq 1 - \frac{dm(m-1)}{\sqrt{2\pi}(R-1)}.\]
\end{remark}
